Probing Classifiers are Unreliable for Concept Removal and Detection

Neural network models trained on text data have been found to encode undesirable linguistic or sensitive concepts in their representation. Removing such concepts is non-trivial because of a complex relationship between the concept, text input, and the learnt representation. Recent work has proposed post-hoc and adversarial methods to remove such unwanted concepts from a model's representation. Through an extensive theoretical and empirical analysis, we show that these methods can be counter-productive: they are unable to remove the concepts entirely, and in the worst case may end up destroying all task-relevant features. The reason is the methods' reliance on a probing classifier as a proxy for the concept. Even under the most favorable conditions for learning a probing classifier when a concept's relevant features in representation space alone can provide 100% accuracy, we prove that a probing classifier is likely to use non-concept features and thus post-hoc or adversarial methods will fail to remove the concept correctly. These theoretical implications are confirmed by experiments on models trained on synthetic, Multi-NLI, and Twitter datasets. For sensitive applications of concept removal such as fairness, we recommend caution against using these methods and propose a spuriousness metric to gauge the quality of the final classifier.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See \refsec{sec:feature_removal_problem} and \ref{sec:feature_removal_expt_main}}
  \item Did you describe the limitations of your work?
    \answerYes{See \refappendix{sec:limitation_of_our_work}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \refappendix{sec:app_broader_impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Our work show failure modes of existing concept removal methods.}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See \refsec{sec:feature_removal_problem}}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See \refappendix{sec:app_probing},\ref{sec:app_inlp_setup_proof} and \ref{sec:app_adv_setup_proof}. }
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See \refappendix{sec:app_expt_setup}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \refappendix{sec:app_expt_setup}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See \refsec{sec:feature_removal_expt_main}, \refappendix{sec:app_expt_setup} and \refappendix{sec:app_additional_results}.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \refappendix{subsec:compute_resource}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See \refsec{sec:feature_removal_expt_main} and \refappendix{sec:app_expt_setup}.}
  \item Did you mention the license of the assets?
    \answerYes{See \refappendix{sec:app_expt_setup}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/apdx_fig1_breakdown.tex <==
\section{Breakdown of \reffig{fig:inlp_pretrained_model}}
\label{sec:fig1a_breakdown}
% \newPT{\rbl{
For greater interpretability, we have added \reffig{fig:inlp_pretrained_model_expand} where we break down \reffig{fig:inlp_pretrained_model} and show the two classifiers separately. \reffig{fig:inlp_pretrained_model_expand_main} shows the profession classifier and its projected points on the classifier line. \reffig{fig:inlp_pretrained_model_expand_prob} shows the slanted gender classifier, the input points, and its projections on the gender classifier. 
% }}


\begin{figure}[t]
\centering
    \begin{subfigure}[h]{.48\textwidth}
        \captionsetup{justification=centering}
        \centering
            \includegraphics[width=\linewidth,height=0.8\linewidth]{figs/Null-Space-Classifier-Illustration-Flip-NeurIPS-Sub-v2-Main.pdf}
            % \includesvg[width=\linewidth,height=0.7\linewidth]{figs/NullSpace-FairClassifier.svg}
    		\caption[]%
            {{\small Clean Pretrained Main-Task (Profession) Classifier}}    
    		\label{fig:inlp_pretrained_model_expand_main}
    \end{subfigure}
\hfill 
  \begin{subfigure}[h]{.48\textwidth}
  \captionsetup{justification=centering}
    \centering
    \includegraphics[width=\linewidth,height=0.8\linewidth]{figs/Null-Space-Classifier-Illustration-Flip-NeurIPS-Sub-v2-Prob.pdf}
		\caption[]%
        {{\small Probing (Gender) Classifier}}    
		\label{fig:inlp_pretrained_model_expand_prob} 
  \end{subfigure}

\caption{\textbf{\reffig{fig:inlp_pretrained_model} Breakdown}: \reffig{fig:inlp_pretrained_model_expand_main} shows the profession classifier and its projected points on the classifier line. \reffig{fig:inlp_pretrained_model_expand_prob} shows the slanted gender classifier, the input points and its projections on the gender classifier. For more details see \refsec{sec:fig1a_breakdown}.}
\label{fig:inlp_pretrained_model_expand}
\end{figure}

==> sections/max_margin_proof.tex <==
\section{A probing classifier does not only learn probing features}
\label{sec:probing_failure}
% \abhinav{we could include both problem with probing and problem with learning a fair/invariant classifier w.r.t. to a particular feature}

\abhinav{Defining the feature and then use the real sentence to motivate. 
Gender and Profession lines}


\abhinav{Merge both precap and story into once paragraph later}
\paragraph{Precap:} A common theme of latent space based removal methods is that they use probing classifier as a proxy for the \sensitive feature they want to remove  in the latent representation. Null-space removal uses the \sensitive feature's probing classifier to remove the information about them from the latent representation. Adversarial removal methods also uses the \sensitive feature's probing classifier to remove the feature but jointly train the main-task classifier.

\paragraph{Story of this section:}
In this section we will show that training a \emph{good} probing classifier and the main-task classifier \emph{individually} is difficult. Hence the individual components of both the removal methods are incorrect i.e probing classifier for null-space and both probing and main-classifier for adversarial removal. Then in the next section we will show that this individual component failure will lead to failure of the removal method put together. We start off, by showing that for any classification task be it probing or main-task classification, it is difficult to learn a \emph{good} classifier which doesn't uses any spuriously correlated feature (\reftheorem{theorem:sufficient_condition}).

% In this section we will we prove a key theoretical result which will help us answer the following question:
% \begin{enumerate}
%     %\item Under what conditions does a main-task classifier starts using features spuriously correlated with main-task feature to make it's prediction?
%     \item Under what conditions does a probing-classifier which is trained to predict the probing label will also use the feature which is spuriously correlated with probing feature?
%     \chenhao{given that the answer to the first question is clearly yes, maybe re-word this part?}
%     \item If our probing-classifier is using unwanted attributes what consequence it will have on the methods like null-space removal and adversarial removal which are used to solve the first problem? Will they fail to remove the unwanted attribute? Or will they have some adverse effect on the desired attribute which are relevant for the main-task?
% \end{enumerate}

%With infinite data, cross-entropy loss is expected to converge to max margin. We also assume linear \amit{what are the linear assumptions}

%We consider a the simple linear setting to study the difficulty in training an invariant-classifier which dont use spurious feature for it prediction. We observed that \refassm{assm:fully_pred_inv} and \refassm{assm:same_side_ls} over the data-distribution, gave us a sufficient condition when the classifier will use spurious feature when trained with max-margin objective. 



% \subsection{Notation and Definitions}
% \paragraph{Notation} Let $(\bm{x}_i,y_i)$ be individual tuple of input and class label respectively in the dataset $\bm{X}$. \amit{better to use D or some other notation for notation since X may be confused with x} Let each datapoint be further composed of both invariant feature (of dimension $d_{inv}$) and spurious part (of dimension $d_{sp}$) i.e $\bm{x}_i=[\bm{x}_{inv},\bm{x}_{sp}]$ where $\bm{x}_{inv}\in \mathbb{R}^{d_{inv}}$ and $\bm{x}_{sp}\in \mathbb{R}^{d_{sp}}$. For the ease of exposition, throughout the paper we assume that we have binary classification task where $y_i\in\{-1,1\}$. We also assume the dataset is zero-centered wherever applicable.

% Let $(\bm{x}_i,y_i)$ be individual input and class label respectively present in the dataset $\bm{X}$. Let each datapoint be further composed of both invariant feature (of dimension $d_{inv}$) and spurious part (of dimension $d_{sp}$) i.e $\bm{x}_i=[\bm{x}_{inv},\bm{x}_{sp}]$ where $\bm{x}_{inv}\in \mathbb{R}^{d_{inv}}$ and $\bm{x}_{sp}\in \mathbb{R}^{d_{sp}}$. Let the class labels $y_i$ be binary taking value from set $\{-1,1\}$ .




% \amit{need to specify it is only for linear}
% \amit{need to justify use of max margin versus cross-entropy}

% Next, we will start with few definitions which will be useful in the exposition of this section.











\subsection{Definition and Assumption}
Following earlier work from \cite{FailureModeOODGen}, we assume a max-margin loss when training the classifier.  Recent work by \cite{GradDescentMaxMargin} shows that under some condition on separable data, a classifier trained using logistic/exponential loss will converge to max-margin classifier given infinite training time. Let $\in\mathcal{D}_{p}$ be the dataset containing inputs $\bm{x}^{i}$ and the corresponding probing feature label $y_{p}^{i}$. Let the encoder $h:\bm{x}\rightarrow \bm{z}$ mapping the input $\bm{x}^{i}$ to latent representation $\bm{z}^{i}$ be frozen when training the linear probing classifier $c_p:\bm{z}\rightarrow y_{p}$. For NLP domain, it's common to use pretrained language model like \cite{devlin-etal-2019-bert} or \cite{roberta19} fine tuned over the main task. Also, let the probing feature label $y_{p}^{i}$ be binary taking values from $\{-1,1\}$. For ease of analysis we make the following assumptions:

\amit{adding some text from Sec 2--check if useful}Let there be probing dataset $\mathcal{D}_{p}$ (possibly different from main task dataset $\mathcal{D}_{m}$) where for every input $\bm{x}^{i}$ we have the probe-label $y^{i}_{p}$ for the feature which we want to probe. The probing method work by training a probing classifier $c_{p}:\bm{z}\rightarrow y_{p}$ which is trained to predict the label $y_{p}$ from the frozen latent representation $\bm{z}$. 

\amit{do we need any other assumption from the previous theory paper? I remember they had 5-6 assumptions}

\begin{assumption}[Disentangled Latent Representation]
\label{assm:disentagled_latent}
The latent representation $\bm{z}$ is disentangled and is of form $[\bm{z}_{m},\bm{z}_{p}]$, where  $\bm{z}_{p}\in \mathbb{R}^{d_{p}}$ is the feature conceptually relevant for probing task prediction and $\bm{z}_{m}\in \mathbb{R}^{d_{m}}$ contains feature conceptually desirable for the main task along with  rest of the feature. Here $d_{m}$ and $d_{p}$ are the dimensions of $\bm{z}_{m}$ and $\bm{z}_{p}$ respectively. Also, let $\bm{z}$ be linearly separable with respect to both binary labels $y_{m}$ and $y_{p}$ taking values from $\{-1,1\}$.
\end{assumption}

% \abhinav{write about the encoder. It could be anything in general. Should we specify this?}
% \abhinav{Define the two datasets, one for probing and one for the main task}.
% \abhinav{write the layer after this is linear}.

Here $\bm{z}_{m}$ and $\bm{z}_{p}$ are spuriously correlated with each other, hence w.r.t. the main-task $\bm{z}_{p}$ is the spurious feature and for the probing task $\bm{z}_{m}$ is the spurious feature. Instead of looking both the task separately, for the ease of exposition in this section we will assume that there is a classification task for which the latent representation $\bm{z}$ is of form $[\bm{z}_{inv},\bm{z}_{sp}]$ where $\bm{z}_{inv}$ is the feature invariant/relevant for the task and $\bm{z}_{sp}$ is spuriously correlated with the $\bm{z}_{inv}$. Also, let $y$ be the corresponding label for this classification task. Later, based on the classifier we are using, we can assign $\bm{z}_{m}$ and $\bm{z}_{p}$ as one of $\bm{z}_{inv}$ or $\bm{z}_{sp}$. Next, based on which feature the classifier is using we define two different categories:



\begin{definition}[Purely-Invariant Classifier] 
\label{def:purely_invariant}
Given a linear classifier of form $c(\bm{z}) = \bm{w}_{inv}\bm{z}_{inv} + \bm{w}_{sp} \bm{z}_{sp} + b$ optimized using max-margin objective. The classifier is called \emph{"purely-invariant"} if it does not use the spurious features $\bm{z}_{sp}$ i.e.,  $\bm{w}_{sp}=\bm{0}$.
\end{definition}



\begin{definition}[Spurious-Using Classifier]
\label{def:spurious_using}
Given a linear classifier of form $c(\bm{z}) = \bm{w}_{inv}\bm{z}_{inv} + \bm{w}_{sp} \bm{z}_{sp} + b$ optimized using max-margin objective. The classifier is called \emph{"spurious-using"} if it  uses the spurious features $\bm{z}_{sp}$ i.e., $\bm{w}_{sp}\neq \bm{0}$.
\end{definition}

\amit{invariant and spurious are not the right keywords for a probing classifier. Perhaps Property-only classifier and Confounded classifier}



In addition, while it may be less surprising that a spurious feature is used if the invariant feature does not give 100\% accuracy,  we show that a spurious feature will be used even if the invariant feature is fully predictive of the label, following ~\cite{FailureModeOODGen}. We formalize it as, 
\begin{assumption}[Invariant Feature Linear Separability]
\label{assm:fully_pred_inv}
The invariant part of the latent representation ($\bm{z}_{inv}$) for every point is linearly separable/fully predictive of the classification task labels $y$, i.e $y^{i}\cdot (\hat{\bm{\epsilon}}_{inv}\cdot \bm{z}_{inv}^{i} + b_{inv}) \geq 1$ for all datapoints $(\bm{x^i},y^{i})$ for some $\hat{\bm{\epsilon}}_{inv}\in \mathbb{R}^{d_{inv}}$.  For the case of zero-centered latent space we have $b_{inv}=0$.
\end{assumption}




% Our first assumption is over the margin points of both side of margin of \emph{purely-invariant} classifier.
% \begin{assumption}[Opposite-Side Linear Separability]
% \label{assm:other_side_ls}
% Let $\bm{X}$ be set of all points in the dataset. Let $\bm{X}^{m,y}$ be the set of margin point of \emph{purely-invariant} classifier (\refdef{def:purely_invariant}) having same class label $(y)$, where $y\in\{-1,1\}$. We assume that there exist a unit vector $\bm{\hat{\epsilon}}_{sp}\in \bm{\mathbb{R}}^{d_{sp}}$ which linearly separates the spurious component of any such pair of margin points, $\bm{x}^{m,-1}\in \bm{X}^{m,-1}$ and $\bm{x}^{m,1}\in \bm{X}^{m,1}$ i.e:
% \begin{equation*}
%     (\bm{\hat{\epsilon}}_{sp} \cdot \bm{x}_{sp}^{m,-1}-b_{sp}) \cdot (\bm{\hat{\epsilon}}_{sp} \cdot  \bm{x}_{sp}^{m,1}-b_{sp}) \leq 0 
% \end{equation*}
% for some $b_{sp}\in \mathbb{R}$. For the case of zero-centered dataset we have $b_{sp}=0$.
% \end{assumption}


In contrast to the fully-predictive invariant feature assumption (\ref{assm:fully_pred_inv}), we only require the spurious feature to be linearly separable for only a very small subset of points in the dataset. Formally,
\begin{assumption}[Spurious Feature Linear Separability]
\label{assm:same_side_ls}
The spurious part of latent representation $(\bm{z}_{sp})$ for the margin points of \emph{purely-invariant} classifier are linearly separable i.e there exist an unit vector $\bm{\hat{\epsilon}}_{sp} \in \bm{\mathbb{R}}^{d_{sp}}$ and $b_{sp}\in \mathbb{R}$ such that $y^{i}(\bm{\hat{\epsilon}}_{sp} \cdot \bm{z}^{i}_{sp} + b_{sp}) > 0$ for every margin point $\bm{x}^{i}$ of the purely-invariant classifier. For the case of zero-centered latent space we have $b_{sp}=0$.
\end{assumption}

\amit{need to justify these assumptions better--I tried below}.
\amit{How common/restrictive is this assumption? good to give examples of datasets that satisfy it (or not)}
\abhinav{we could use the figure in the motivation figure to demonstrate an this condition in 1D}



\begin{figure}[t]
\centering

  \begin{subfigure}[h]{.32\textwidth}
    \centering
        \includegraphics[width=\linewidth,height=0.7\linewidth]{figs/ConvergenceProblem-Illustration.png}
		\caption[]%
        {{\small Spuriousness Condition}}    
		\label{fig:illstrate_conv}
  \end{subfigure}
%   \hfill
  
%   \medskip


\caption{\textbf{Failure Mode of ERM trained with max-margin} \chenhao{Explain more ... I am not sure what you try to say with this figure and the text is not legible}} 
\label{fig:conv_problem_illustration}
\end{figure}



\reffig{fig:illstrate_conv} illustrates the \refassm{assm:same_side_ls} and \ref{assm:fully_pred_inv} when the invariant and spurious feature are both $1$-dimensional. We can see that the invariant feature (x-axis) is fully predictive of the label colored in red and green. The 4 points marked in bold in the first and third quadrant are the margin points of the purely invariant classifier. We can observe that the spurious component of these margin point are linearly separable. For the latent space distribution in \ref{fig:illstrate_conv} of the points all the assumption mentioned above are satisfied and the max-margin classifier is also \emph{spurious-using}. We will formalize this result in the next-section.

%For a classifier trained using max-margin objective to use the spurious feature, all the positive labels should lie in the green region and all the negative ones in the red. Here the \ref{assm:fully_pred_inv} is satisfied since the invariant feature is fully predictive of the labels. In the second and fourth quadrant ($Smin$) the feasible region of data-points are guided by the the location of the margin points present in the first and third quadrant $Smaj$. For the positive labels (green region), none of datapoint in the fourth quadrant could have invariant feature value less than the margin point's invariant value in the first quadrant and similarly for the negative region. This constraint is summarized in \refassm{assm:same_side_ls} for higher dimensional feature.







\subsection{Sufficient Condition for \emph{Spurious-Using} Classifier}


Now we are ready to state the first key result where we give sufficient condition for learning a \emph{spurious-using} classifier. We will show that given \refassm{assm:disentagled_latent}, \ref{assm:fully_pred_inv} and \ref{assm:same_side_ls} holds, we can always construct a \emph{spurious-using} classifier given any \emph{purely-invariant} classifier. which has a margin greater than or equal to the margin of \emph{purely-invariant} one. Thus, this will imply that the optimal linear-classifier trained using max-margin objective is always \emph{spurious-using}.

\begin{theorem}[Sufficient Condition]
\label{theorem:sufficient_condition}
Assuming \ref{assm:disentagled_latent}, \ref{assm:fully_pred_inv} and \ref{assm:same_side_ls}, the optimal linear-classifier when trained using max-margin objective will always be spurious-using (\refdef{def:spurious_using}).
\end{theorem}
\begin{proof}[Proof Sketch]
Since the invariant part of latent representation is fully predictive (\refassm{assm:fully_pred_inv}) we always have a purely-invariant classifier i.e $c_{inv}(\bm{z})=\bm{w}_{inv}\cdot \bm{z}_{inv}$. Given this, we can construct a spurious using classifier $(c_{sp}(\bm{z}))$ by perturbing the parameters of the fully-predictive one. We need to show that the perturbed classifier is fully predictive of task label and has bigger margin than $c_{inv}(\bm{z})$ . For the margin points of the purely invariant point since they are also linearly separable in spurious dimension from \refassm{assm:same_side_ls}, a combination of the purely invariant classifier and this spurious direction i.e $c_{sp}(\bm{z})=\alpha (\bm{w}_{inv}\cdot \bm{z}_{inv}) + \sqrt{1-\alpha^{2}}\norm{\bm{w}_{inv}}(\hat{\bm{\epsilon}}_{sp}\cdot \bm{z}_{sp})$ is still linearly separable and has bigger margin for some $\alpha\in[0,1)$. Next for every non-margin points we show that we can always choose an $\alpha\in [0,1)$ such that we have bigger margin than the purely invariant classifier. Thus we are able to construct a classifier which has bigger margin than $c_{inv}(\bm{z})$ and is spurious-using.
\end{proof}

\chenhao{this makes sense! I do not think it should be here, but we should say how this theorem adds to existing literature.}

\amit{Need a proof sketch here, and for all other theorems. A paragraph that describes the proof idea in words}











\reftheorem{theorem:sufficient_condition} shows that  \refassm{assm:disentagled_latent}, \ref{assm:fully_pred_inv} and \ref{assm:same_side_ls} is sufficient for obtaining a \emph{spurious-using} classifier. Next we are ready to state the second part of our result where we show the necessary condition of learning a \emph{spurious-using} classifier.

\amit{invariant feature being single dimension is a strong assumption. In the writing, let's just claim we have a sufficient condition. Necessary only for a special case}
\begin{proposition}[Necessary Condition]
\label{theorem:necessary_condition} Given \refassm{assm:disentagled_latent} and \ref{assm:fully_pred_inv} holds and the invariant feature is one-dimension i.e $z_{inv},w_{inv}\in \mathbb{R}$. Then the optimal classifier obtained after optimizing the max-margin objective is spurious-using iff \refassm{assm:same_side_ls} holds.
\end{proposition}
\begin{proof}[Proof Sketch]

\end{proof}

%\reftheorem{theorem:sufficient_condition} helps us answer the first two question with which we started this section. Given all the assumption is satisfied, the main-task classifier where $\bm{z}_{m}$ is the relevant feature and $\bm{z}_{p}$ is the spurious feature will also use spurious feature $\bm{z}_{p}$ along with $\bm{z}_{m}$ for its final prediction. This results give us a realization that even under very simplistic setting where the main classifier is linear,  invariant features in the latent space are $100\%$ predictive and the spurious feature are only linearly separable on a very small subset of dataset, the main-task classifier still uses unwanted features. This calls for developing methods which could make a classifier invariant to these unwanted/spurious feature.

\reftheorem{theorem:sufficient_condition} helps us answer the first question with which we started this section. For the probing classifier where $\bm{z}_{p}$ is the conceptually desired/invariant feature and $\bm{z}_{m}$ is the spurious feature, the probing task will also use spurious feature $\bm{z}_{m}$ along with $\bm{z}_{p}$ for its prediction. This says that we cannot learn a correct probing classifier which could have adverse affect on the claims of the probing based removal method which uses probing classifier as a proxy for the feature they want to remove. We demonstrate the failure modes of the probing based removal method in next section (\ref{sec:feature_removal_problem}).
\abhinav{Should we also include the problem with probing result?}
\abhinav{This could come in first second and the expt section}



